Physician Detection of Clinical Harm in Machine Translation: Quality Estimation Aids in Reliance and Backtranslation Identifies Critical Errors

A major challenge in the practical use of Machine Translation (MT) is that users lack guidance to make informed decisions about when to rely on outputs. Progress in quality estimation research provides techniques to automatically assess MT quality, but these techniques have primarily been evaluated in vitro by comparison against human judgments outside of a specific context of use. This paper evaluates quality estimation feedback in vivo with a human study simulating decision-making in high-stakes medical settings. Using Emergency Department discharge instructions, we study how interventions based on quality estimation versus backtranslation assist physicians in deciding whether to show MT outputs to a patient. We find that quality estimation improves appropriate reliance on MT, but backtranslation helps physicians detect more clinically harmful errors that QE alone often misses.

==> emnlp2023_latex/backuptext.tex <==

\ignore{
Decades of research have provided a wealth of techniques to automatically evaluate and estimate the quality of machine translation (MT) \cite{}. However, these techniques are primarily used by MT researchers and developers, driving benchmarks and deployment \cite{}, and to support the workflow of professional translators in post-editing tasks \cite{}. By contrast, online translation tools only display input and output texts and do not provide users with any information on the quality of the output.  This is particularly problematic in high-stakes use cases, such as in hospitals and courtrooms where MT is increasingly used in the absence of interpreters \cite{}. In those cases, users are only proficient in either the source or the target language and are left to develop their own strategies to decide how to rely on potentially imperfect MT output. This has had harmful consequences such as asylum applications denied on the basis of an MT error, wrongful arrests, or clinically incorrect translations \cite{vieira2021understanding}.

This work contributes a human-centered approach to measuring how interventions based on folk strategies vs. state-of-the-art quality estimation techniques impact how U.S.-based physicians rely on machine translation to communicate discharge instructions to patients who do not speak English. \mc{Motivate novelty: in vivo vs. in vitro evaluation, BT is largely considered misleading, usefulness of QE is not clear (little evidence available, Bojar studies give contradicting results.} We contribute evaluation data and a study design informed by the real-world needs of physicians uncovered in prior work, as we will discuss in Section~\ref{sec:usecase}. Most saliently, \citet{mehandru2022reliable} found that clinicians routinely use MT to communicate with patients with limited English proficiency (LEP), yet they struggle to calibrate their assessment of MT errors when they have no knowledge of the output language.

%Cross-lingual communication between physicians and limited English proficiency (LEP) patients is crucial in delivering high quality care. Machine translation (MT) systems, most notably Google Translate, are often deployed in clinical settings when access to medical interpreters remain limited \cite{mehandru2022reliable}. While clinicians have been found to leverage such systems; they have struggled to calibrate errors in machine-generated translations when they have no knowledge of the target language. 

In an experiment with 60 English-speaking physicians, we test how one of two interventions, back translation and quality estimation, can help physicians identify mistranslations in MT outputs (Figure~\ref{fig:example}).\mc{We need an example to illustrate our task on page 1: source/MT output/reference/BT/QE}  We find that both interventions improve physicians ability to assess clinical risk and improved their confidence in their decisions.
}


\paragraph{XAI} Despite the recent explosion of research into explainability techniques for AI/NLP, it remains unclear whether they can deliver on the promise of helping users calibrate their trust in systems, and decide how to appropriately rely on imperfect outputs in practice. This is in part due to a gap between the proxy evaluations that guide system development and actual real world applications \cite{narayanan2018humans} \mc{cite Jordan's tutorial, Bucina, Doshi-Velez and Kim, }. In this work, we study a system that is already used by millions on a daily basis\footnote{\url{https://blog.google/products/translate/one-billion-installs/}} for a real task that physicians cannot perform alone without AI help \citep{mehandru2022reliable}. We evaluate the impact of two different types of explanations on physician reliance and trust in the system. These explanation techniques are not faithful, as they do not provide insights on how the MT system produced an output; Instead they provide the actionable information that users ask for in needfinding studies: how good is a given translation?

\section{From Experimental Design}

For the baseline, physicians were asked to read a given discharge instruction, and were shown the following definition of Google Translate: 

\textit{Google Translate is a translation system that allows users to automatically translate text from one language to another. Automatic translation systems like Google Translate; however, can sometimes make errors.}\mc{Do we need this in the main paper? can this be moved to the appendix?}

After reading the discharge instruction, physician participants were told that a sentence from the note was translated into Chinese by Google Translate. Participants were then asked a binary question (yes or no) if they would give the translation to a patient who only reads Chinese assuming a medical interpreter had already reviewed the instruction with the monolingual Chinese patient. Participants were also asked how confident they were in their decision to give, or not give, the translation to a patient on a five-point Likert scale (1= Not Confident and 5= Very Confident). \sa{Add citation}

After the baseline condition, physicians received one of two treatment interventions: 1) a back translation condition, and 2) a quality estimation condition. Similar to the baseline condition, the physician participants were asked whether they would give the Chinese translation to a patient who only reads Chinese and their level of confidence in that decision. Participants were instructed to respond to questions barring a lawsuit and regulatory requirements around showing an imperfect translation to a Chinese-speaking patient, and instead were asked to focus on patient comprehension of discharge instructions as it pertains to clinical outcomes. Unlike the baseline condition, in both treatment conditions, participants are asked about patient comprehension, specifically if a monolingual Chinese patient were to read the generated Chinese translation, how much the patient would understand the discharge instruction sentence on a 5-point Likert scale (1= Patient would understand none of the meaning and 5= Patient would understand all of the meaning).


==> emnlp2023_latex/old_results/old_results.tex <==
%% Old results

% \subsection{prelim analysis}
% Both interventions improved participants' ability to detect clinically harmful translations (Figure~\ref{fig:accuracy}) and increased their confidence in their decisions (Figure~\ref{fig:confidence}). The percentage of correct answer improves by about 10\% over the baseline in the QE condition and 5\% in the BT condition. 

% Further analysis suggests that the two interventions provide complementary feedback. In the BT condition, people got really good at detecting errors, they on average caught 92\% of errors, vs QE that caught 70\% and baseline that caught about 62\%. In the QE condition, people got really good at detecting the correct translations, they on average correctly identified a correct translation 91\% of the time, vs. BT 66\% and baseline about 70\% (Figure~\ref{fig:errorcategory}). 

% \begin{figure}[h]
% \centering
% \includegraphics[width=\linewidth]{emnlp2023-latex/figs/accepted_count.png}
% \caption{Physicians on average accept translations more under the QE intervention.} \label{fig:accept}
% \end{figure}


% \begin{figure}[h]
% \centering
% \includegraphics[width=\linewidth]{emnlp2023-latex/figs/correc_confidence.png}
% \caption{BT and QE interventions improve physicians ability to correctly detect clinically harmful translations. Error bars represent standard error. } \label{fig:accuracy}
% \end{figure}


% \begin{figure}[h]
% \centering
% \includegraphics[width=\linewidth]{emnlp2023-latex/figs/confidence.png}
% \caption{BT and QE interventions improve physicians confidence in their assessment of clinical risk. Error bars represent standard error.} \label{fig:confidence}
% \end{figure}


% \begin{figure*}[h]
% \centering
% \includegraphics[width=\linewidth]{emnlp2023-latex/figs/changebaseline.png}
% \caption{Both interventions lead to a significant improvement in user accuracy over baseline with significantly higher confidence.} \label{fig:accuracy}
% \end{figure*}


% \begin{figure*}[h]
% \centering
% \includegraphics[width=\linewidth]{emnlp2023-latex/figs/correctVsincorrect.png}
% \caption{Backtranslation enables better detection of errors whereas QE enables the physicians to pick more correct translations, suggesting complementary advantages of both interventions. \sa{typo in right diagram and also numbers need fixing}} \label{fig:errorcategory}
% \end{figure*}

==> emnlp2023_latex/sleepingkittens.tex <==
% For placing
\begin{figure*}[t]
\begin{subfigure}{0.45\linewidth}
\centering
\includegraphics[width=0.8\linewidth]{emnlp2023-latex/figs/accuracy_yes_physican.png}
\caption{Correct Identification of Adequate Translations}
\end{subfigure}
\begin{subfigure}{0.45\linewidth}
\centering
\includegraphics[width=0.8\linewidth]{emnlp2023-latex/figs/accuracy_no_physican.png}
\caption{Correct Identification of Inadequate Translations}
\end{subfigure}
\caption{The QE treatment group had an overall higher accuracy in correctly relying on MT systems when translations were adequate whereas the BT treatment group had a higher accuracy in judging inadequate translations. \\ ns: not significant;$**$: significant with p-value of 0.01; $****$: p-value of 0.0001.} 
 % \vspace{-0.5cm}
 \label{fig:physician_reliance}
\end{figure*}


\begin{figure}[h]
\begin{subfigure}{0.9\linewidth}
\centering
\includegraphics[width=\linewidth]{emnlp2023-latex/figs/accuracy_overall_physican.png}
\end{subfigure}
\caption{The QE treatment group relies on MT more accurately than the BT group. The difference in Physician accuracy between the two treatment groups is statistically significant.
% \mc{The 2nd sentence needs to be more specific because there is only 1 comparison that is significant in the graph.} \sa{Updated}
ns: not significant; $**$: significant with p-value of 0.01.} \label{fig:overall_physician}
\end{figure}


\begin{figure*}[t]
\begin{subfigure}{0.45\linewidth}
\centering
\includegraphics[width=0.8\linewidth]{emnlp2023-latex/figs/accuracy_yes_physican.png}
\caption{Correct Identification of Adequate Translations}
\end{subfigure}
\begin{subfigure}{0.45\linewidth}
\centering
\includegraphics[width=0.8\linewidth]{emnlp2023-latex/figs/accuracy_no_physican.png}
\caption{Correct Identification of Inadequate Translations}
\end{subfigure}
\caption{The QE treatment group had an overall higher accuracy in correctly relying on MT systems when translations were adequate whereas the BT treatment group had a higher accuracy in judging inadequate translations. \\ ns: not significant;$**$: significant with p-value of 0.01; $****$: p-value of 0.0001.} 
 % \vspace{-0.5cm}
 \label{fig:physician_reliance}
\end{figure*}

